Fast, Sound and Effectively Complete Dynamic Race Prediction

Writing concurrent programs is highly error-prone due to the nondeterminism in interprocess communication. The most reliable indicators of errors in concurrency are data races, which are accesses to a shared resource that can be executed consecutively. We study the problem of predicting data races in lock-based concurrent programs. The input consists of a concurrent trace $t$, and the task is to determine all pairs of events of $t$ that constitute a data race. The problem lies at the heart of concurrent verification and has been extensively studied for over three decades. However, existing polynomial-time sound techniques are highly incomplete and can miss many simple races. In this work we develop M2: a new polynomial-time algorithm for this problem, which has no false positives. In addition, our algorithm is complete for input traces that consist of two processes, i.e., it provably detects all races in the trace. We also develop sufficient conditions for detecting completeness dynamically in cases of more than two processes. We make an experimental evaluation of our algorithm on a standard set of benchmarks taken from recent literature on the topic. Our tool soundly reports thousands of races and misses at most one race in the whole benchmark set. In addition, our technique detects all racy memory locations of the benchmark set. Finally, its running times are comparable, and often smaller than the theoretically fastest, yet highly incomplete, existing methods. To our knowledge, M2 is the first sound algorithm that achieves such a level of performance on both running time and completeness of the reported races.

==> dc_example.tex <==
\section{An Example of a Difficult Race}\label{sec:dc_example}

As we have seen in \cref{SEC:INTRO}, in order for the work of \cite{Roemer18} to detect a race $(\Event_1, \Event_2)$, the following three phases need to succeed.
\begin{compactenum}
\item[\emph{Phase~1}.] The $\DC$ partial order is constructed, and we must have $\Event_1\not\leq_{\DC} \Event_2$, i.e., the two events must not be $\DC$ ordered.
\item[\emph{Phase~2}.] A constraint graph $G$ is constructed which strengthens some $\DC$-orderings by introducing extra edges in $G$.
Here $G$ must remain acyclic, as otherwise it is reported that $(\Event_1, \Event_2)$ is not a race.
Intuitively, a cycle in $G$ implies that the algorithm fails to construct a witness trace.
\item[\emph{Phase~3}.] A witness trace $\Trace^*$ is built backwards, by starting with $\Event_1,\Event_2$ and prepending events to $\Trace^*$ in a greedy way as dictated by $G$.
Here $\Trace^*$ must be constructed without violating lock-semantics, as otherwise the algorithm fails to construct a valid witness and reports that $(\Event_1, \Event_2)$ is not a race.
\end{compactenum}

\cref{subfig:motivating_incomplete1} and \cref{subfig:motivating_incomplete2} in \cref{SEC:INTRO} show two examples where the above process fails in Phase~1 and Phase~2, respectively.
The authors of \cite{Roemer18} have identified a complicated example of $7$ processes where their algorithm fails in Phase~3.
\cref{subfig:dc_example} shows the example adapted in our setting, and the task is to detect the race $(\Event_{25}, \Event_{32})$.
We also note that the race is missed by each of the other techniques we have used in this work, namely $\HB$, $\WCP$, and $\SHB$.
For simplicity, we make the following conventions.
\begin{compactenum}
\item We assume a salient write event to each memory location that precedes every event shown in the trace of \cref{subfig:dc_example}.
\item We use the command $\Sync(s_i)$ to denote the (atomic) sequence $\Acquire(s_i),\Read(x_i), \Write(x_i), \Release(s_i)$.
Hence, $\Sync$ events on the same variable are totally ordered.
\end{compactenum}


We have verified that our algorithm $\RaceFunction$ detects the race $(\Event_{25}, \Event_{32})$ and constructs the witness trace shown in \cref{subfig:dc_example_witness}.
It is a non-trivial race, the detection of which requires the reordering of many events.
This is an interesting example where the exact operation of \cref{line:insert_and_close} of $\RaceDecision$ (\cref{algo:racedecision}) is crucial: after resolving a conflict arbitrarily, by inserting the edge $\ov{\Event}_1\to \ov{\Event}_2$ in $Q$, a closure computation must be performed. Without the closure computation, the algorithm would fail to catch this race.


\input{figures/dc_example}

==> experimental_table.tex <==
\begin{table}
\tiny
\centerline{
\begin{tabular}{|c|c|c|||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|c|}
\hline
\textbf{Benchmark} & $\boldsymbol{k}$ & $\boldsymbol{n}$ & \multicolumn{3}{c||}{$\boldsymbol{\HB}$}& \multicolumn{3}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{3}{c||}{$\boldsymbol{\SHB}$}& \multicolumn{3}{c||}{$\boldsymbol{\DC}$}& \multicolumn{4}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
& & &$\boldsymbol{\PR}$ & $\boldsymbol{\FalsePositives}$ & $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\PR}$ & $\boldsymbol{\FalsePositives}$ & $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\PR}$ & $\boldsymbol{\FalsePositives}$ & $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\PR}$ & $\boldsymbol{\FalsePositives}$ & $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\Races}$ & D-Races & D-Rev & $\boldsymbol{\FalseNegativesBound}$ \\
\hline
\hline
\texttt{array} & 2 & 50 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -1\\
\hline
\texttt{critical} & 3 & 57 & 8 & 0 & 0 & 8 & 0 & 0 & 8 & 0 & 0 & 8 & 0 & 0 & 8 & 0 & -1 & -1\\
\hline
\texttt{airtickets} & 2 & 122 & 6 & 0 & 0 & 6 & 0 & 0 & 6 & 0 & 0 & 6 & 0 & 0 & 6 & 0 & -1 & -1\\
\hline
\texttt{account} & 3 & 133 & 18 & 15 & 0 & 18 & 15 & 0 & 3 & 0 & 0 & 22 & 19 & 0 & 3 & 0 & -1 & -1\\
\hline
\texttt{pingpong} & 4 & 137 & 16 & 10 & 0 & 16 & 10 & 0 & 6 & 0 & 0 & 16 & 10 & 0 & 6 & 0 & -1 & -1\\
\hline
\texttt{bbuffer} & 2 & 330 & 9 & 0 & 0 & 9 & 0 & 0 & 9 & 0 & 0 & 9 & 0 & 0 & 9 & 0 & -1 & -1\\
\hline
\texttt{mergesort} & 4 & 3.0K & 70 & 67 & 50 & 70 & 67 & 50 & 2 & 0 & 51 & 262 & 209 & 0 & 53 & 48 & -1 & -1\\
\hline
\texttt{bubblesort} & 10 & 4.0K & 3142 & 2338 & 105 & 3150 & 2338 & 97 & 802 & 0 & 107 & 4068 & 3159 & 0 & 909 & 107 & -1 & -1\\
\hline
\texttt{raytracer} & 2 & 16K & 1335 & 668 & 0 & 1335 & 668 & 0 & 667 & 0 & 0 & 1337 & 670 & 0 & 667 & 0 & -1 & -1\\
\hline
\texttt{ftpserver} & 10 & 48K & 186 & 99 & 29 & 186 & 99 & 29 & 87 & 0 & 29 & 621 & 512 & 7 & 116 & 0 & -1 & -1\\
\hline
\texttt{moldyn} & 2 & 143K & 327846 & 318788 & 0 & 327846 & 318788 & 0 & 9058 & 0 & 0 & 327846 & 318788 & 0 & 9058 & 0 & -1 & -1\\
\hline
\texttt{derby} & 3 & 1.0M & 145 & 106 & 0 & 145 & 106 & 0 & 39 & 0 & 0 & 7433 & 7394 & 0 & 39 & 0 & -1 & -1\\
\hline
\texttt{jigsaw} & 12 & 3.0M & 27 & 9 & 2 & 30 & 10 & 0 & 18 & 0 & 2 & 1576 & 1556 & 0 & 20 & 0 & -1 & -1\\
\hline
\texttt{bufwriter} & 5 & 11M & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & 11 & 0 & -1 & -1\\
\hline
\texttt{cryptorsa} & 6 & 43M & 6 & 1 & 21 & 8 & 1 & 19 & 5 & 0 & 21 & -1 & -1 & -1 & 26 & 0 & -1 & -1\\
\hline
\texttt{eclipse} & 14 & 90M & -1 & -1 & -1 & -1 & -1 & -1 & 663 & 0 & 235 & 52745 & 51982 & 135 & 898 & 30 & -1 & -1\\
\hline
\texttt{xalan} & 6 & 122M & -1 & -1 & -1 & -1 & -1 & -1 & 89 & 0 & 8 & -1 & -1 & -1 & 97 & 0 & -1 & -1\\
\hline
\texttt{lusearch} & 7 & 217M & -1 & -1 & -1 & -1 & -1 & -1 & 360 & 0 & 0 & -1 & -1 & -1 & 360 & 0 & -1 & -1\\
\hline
\end{tabular}
}
\caption{FIX}
\label{tab:experimental}
\end{table}



\begin{table}
\tiny
\centerline{
\begin{tabular}{|c|c|c|||c||c||c||c||c|c|c|}
\hline
\textbf{Benchmark} & $\boldsymbol{k}$ & $\boldsymbol{n}$ & \multicolumn{1}{c||}{$\boldsymbol{\HB}$}& \multicolumn{1}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{1}{c||}{$\boldsymbol{\SHB}$}& \multicolumn{1}{c||}{$\boldsymbol{\DC}$}& \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
& & &$\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\Races}$ & D-Races & D-Rev\\
\hline
\hline
\texttt{array} & 2 & 50 & 0 & 0 & 0 & 0 & 0 & 0 & -1\\
\hline
\texttt{critical} & 3 & 57 & 0 & 0 & 0 & 0 & 8 & 0 & -1\\
\hline
\texttt{airtickets} & 2 & 122 & 0 & 0 & 0 & 0 & 6 & 0 & -1\\
\hline
\texttt{account} & 3 & 133 & 0 & 0 & 0 & 0 & 3 & 0 & -1\\
\hline
\texttt{pingpong} & 4 & 137 & 0 & 0 & 0 & 0 & 6 & 0 & -1\\
\hline
\texttt{bbuffer} & 2 & 330 & 0 & 0 & 0 & 0 & 9 & 0 & -1\\
\hline
\texttt{mergesort} & 4 & 3.0K & 50 & 50 & 51 & 0 & 53 & 48 & -1\\
\hline
\texttt{bubblesort} & 10 & 4.0K & 105 & 97 & 107 & 0 & 909 & 107 & -1\\
\hline
\texttt{montecarlothirtieth} & 2 & 10K & 1 & 1 & 1 & 1 & 1726 & 0 & 0\\
\hline
\texttt{raytracer} & 2 & 16K & 0 & 0 & 0 & 0 & 667 & 0 & -1\\
\hline
\texttt{ftpserver} & 10 & 48K & 29 & 29 & 29 & 7 & 116 & 0 & -1\\
\hline
\texttt{moldyn} & 2 & 143K & 0 & 0 & 0 & 0 & 9058 & 0 & -1\\
\hline
\texttt{derby} & 3 & 1.0M & 0 & 0 & 0 & 0 & 39 & 0 & -1\\
\hline
\texttt{jigsaw} & 12 & 3.0M & 2 & 0 & 2 & 0 & 20 & 0 & -1\\
\hline
\texttt{cryptorsa} & 6 & 43M & 21 & 19 & 21 & 0 & 26 & 0 & -1\\
\hline
\texttt{eclipse} & 14 & 90M & -1 & -1 & 235 & 135 & 898 & 30 & -1\\
\hline
\texttt{xalan} & 6 & 122M & -1 & -1 & 8 & 3 & 97 & 0 & -1\\
\hline
\texttt{lusearch} & 7 & 217M & -1 & -1 & 0 & 0 & 360 & 0 & -1\\
\hline
\end{tabular}
}
\caption{FIX}
\label{tab:experimental_vc}
\end{table}






\begin{table}
\tiny
\centerline{
\begin{tabular}{|c|c|c|||c||c||c||c|c||c|c|c|}
\hline
\textbf{Benchmark} & $\boldsymbol{k}$ & $\boldsymbol{n}$ & \multicolumn{1}{c||}{$\boldsymbol{\HB}$}& \multicolumn{1}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{1}{c||}{$\boldsymbol{\SHB}$} &\multicolumn{2}{c|}{$\boldsymbol{\DC}$}& \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
& & &$\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\FalseNegatives}-DC$ & \boldsymbol{\FalseNegatives}-Vind & $\boldsymbol{\Races}$ & D-Races & D-Rev\\
\hline
\hline
\texttt{array} & 2 & 50 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1\\
\hline
\texttt{critical} & 3 & 57 & 0 & 0 & 0 & 0 & 0 & 8 & 0 & -1\\
\hline
\texttt{airtickets} & 2 & 122 & 0 & 0 & 0 & 0 & 0 & 6 & 0 & -1\\
\hline
\texttt{account} & 3 & 133 & 0 & 0 & 0 & 0 & 0 & 3 & 0 & -1\\
\hline
\texttt{pingpong} & 4 & 137 & 0 & 0 & 0 & 0 & 0 & 6 & 0 & -1\\
\hline
\texttt{bbuffer} & 2 & 330 & 0 & 0 & 0 & 0 & 0 & 9 & 0 & -1\\
\hline
\texttt{mergesort} & 4 & 3.0K & 50 & 50 & 51 & 0 & 0 & 53 & 48 & -1\\
\hline
\texttt{bubblesort} & 10 & 4.0K & 105 & 97 & 107 & 0 & 434 & 909 & 107 & -1\\
\hline
\end{tabular}
}
\caption{FIX}
\label{tab:experimental_vc_vindicate_dc}
\end{table}











%\begin{table}
%\small
%\begin{tabular}{|c|c|c|||c|c|c|c||c|c|c|c||c|c|c|}
%\hline
%\textbf{Benchmark} & $\boldsymbol{k}$ & $\boldsymbol{n}$ & \multicolumn{4}{c||}{$\boldsymbol{\HB}$} & \multicolumn{4}{c||}{$\boldsymbol{\WCP}$} & \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
%\hline
%& & &  $\boldsymbol{\PR}$ & $\boldsymbol{\FalsePositives}$ & $\boldsymbol{\FalseNegatives}$ &  $\boldsymbol{\Time}$ &  $\boldsymbol{\PR}$ & $\boldsymbol{\FalsePositives}$ & $\boldsymbol{\FalseNegatives}$ & $\boldsymbol{\Time}$ &  $\boldsymbol{\Races}$ & $\boldsymbol{\FalseNegativesBound}$ & $\boldsymbol{\Time}$ \\
%\hline
%\hline
%\texttt{array} & 2 & 50 & 0 & 0 & 0 & 0.40s & 0 & 0 & 0 & 0.30s & 0 & 0 & 0.13s\\
%\hline
%\texttt{critical} & 3 & 57 & 8 & 0 & 0 & 0.28s & 8 & 0 & 0 & 0.28s & 8 & 0 & 0.11s\\
%\hline
%\texttt{airtickets} & 2 & 122 & 6 & 0 & 0 & 0.31s & 6 & 0 & 0 & 0.31s & 6 & 0 & 0.09s\\
%\hline
%\texttt{account} & 3 & 133 & 18 & 15 & 0 & 0.30s & 18 & 15 & 0 & 0.30s & 3 & 0 & 0.10s\\
%\hline
%\texttt{pingpong} & 4 & 137 & 16 & 10 & 0 & 0.31s & 16 & 10 & 0 & 0.34s & 6 & 0 & 0.10s\\
%\hline
%\texttt{bbuffer} & 2 & 330 & 9 & 0 & 0 & 0.32s & 9 & 0 & 0 & 0.31s & 9 & 0 & 0.11s\\
%\hline
%\texttt{mergesort} & 4 & 3.0K & 70 & 67 & 50 & 0.48s & 70 & 67 & 50 & 0.43s & 53 & 0 & 0.15s\\
%\hline
%\texttt{bubblesort} & 10 & 4.0K & 3142 & 2338 & 105 & 2.17s & 3150 & 2338 & 97 & 1.74s & 909 & 0 & 2.14s\\
%\hline
%\texttt{raytracer} & 2 & 16K & 1335 & 668 & 0 & 3.14s & 1335 & 668 & 0 & 1.62s & 667 & 0 & 0.24s\\
%\hline
%\texttt{ftpserver} & 10 & 48K & 186 & 99 & 29 & 2.61s & 186 & 99 & 29 & 2.48s & 116 & 0 & 1.79s\\
%\hline
%\texttt{moldyn} & 2 & 143K & 331621 & 322563 & 0 & 10m4s & 331621 & 322563 & 0 & 3m30s & 9058 & 0 & 0.92s\\
%\hline
%\texttt{derby} & 3 & 1.0M & 145 & 106 & 0 & 41.44s & 145 & 106 & 0 & 21.82s & 39 & 0 & 7.15s\\
%\hline
%\texttt{jigsaw} & 12 & 3.0M & 27 & 9 & 2 & 1m10s & 30 & 10 & 0 & 25.58s & 20 & 0 & 12.80s\\
%\hline
%\texttt{montecarlo} & 2 & 7.0M & - & - & - & TO & - & - & - & TO & >1e6 & - & TO \\
%\hline
%\texttt{bufwriter} & 5 & 11M & 11 & 0 & 0 & 2m32s & 11 & 0 & 0 & 3m2s & 11 & 0 & 2m10s\\
%\hline
%\texttt{cryptorsa} & 6 & 43M & 6 & 1 & 21 & 6m44s & 6 & 1 & 21 & 2m45s & 26 & 0 & 2m36s\\
%\hline
%\texttt{eclipse} & 14 & 90M & 673 & 10 & 235 & 1h37m & 711 & 22 & 209 & 15m20s & 898 & 1 & 1h58m\\
%\hline
%\texttt{xalan} & 6 & 122M & 144 & 54 & 7 & 22m2s & 155 & 61 & 3 & 8m47s & 97 & 0 & 7m56s\\
%\hline
%\texttt{lusearch} & 7 & 217M & - & - & - & TO & - & - & - & TO & 360 & 0 & 7m36s\\
%\hline
%\end{tabular}
%\caption{Experimental comparison of reported races and running time between $\HB$, $\WCP$ and the $\RaceFunction$ algorithm proposed in this paper.}
%\label{tab:experimental}
%\end{table}

==> experimental_table_distances.tex <==
\begin{table}
\small
\centerline{
\begin{tabular}{|c||c|c|c|}
\hline
\textbf{Benchmark} & \textbf{Mean Distance} & \textbf{Max Distance}\\
\hline
\hline
%\texttt{array} & 0 & 0\\
%\hline
%\texttt{critical} & 10 & 16\\
%\hline
%\texttt{airtickets} & 17 & 60\\
%\hline
%\texttt{account} & 10 & 11\\
%\hline
%\texttt{pingpong} & 46 & 97\\
%\hline
%\texttt{bbuffer} & 139 & 214\\
%\hline
%\texttt{mergesort} & 939 & 1.0K\\
%\hline
%\texttt{bubblesort} & 1.0K & 3.0K\\
%\hline
%\texttt{raytracer} & 382 & 880\\
%\hline
\texttt{ftpserver} & 939 & 12K\\
%\hline
%\texttt{moldyn} & 3.0K & 10K\\
%\hline
%\texttt{derby} & 434 & 3.0K\\
\hline
\texttt{jigsaw} & 1.0K & 4.0K\\
%\hline
%\texttt{bufwriter} & 42 & 130\\
\hline
\texttt{cryptorsa} & 144K & 391K\\
\hline
\texttt{eclipse} & 11M & 53M\\
\hline
\texttt{xalan} & 2.0K & 43K\\
\hline
\texttt{lusearch} & 44M & 125M\\
\hline
\end{tabular}
}
\caption{distances}
\label{tab:distances}
\end{table}

==> experimental_table_locs.tex <==
\begin{table}
\small
\centerline{
\begin{tabular}{|c||c|c|c|c|c|}
\hline
\textbf{Benchmark} &$\boldsymbol{\HB}$& $\boldsymbol{\WCP}$& $\boldsymbol{\DC}$& $\boldsymbol{\SHB}$& $\boldsymbol{\RaceFunction}$\\
\hline
\hline
%\texttt{array} & 0 & 0 & 0 & 0 & 0\\
%\hline
%\texttt{critical} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{airtickets} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{account} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{pingpong} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{bbuffer} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{mergesort} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{bubblesort} & 25 & 25 & 25 & 25 & 25\\
%\hline
%\texttt{raytracer} & 3 & 3 & 3 & 3 & 3\\
%\hline
\texttt{ftpserver} & 51 & 51 & 51 & 51 & 54\\
\hline
%\texttt{moldyn} & 2 & 2 & 2 & 2 & 2\\
%\hline
%\texttt{derby} & 15 & 15 & 15 & 15 & 15\\
%\hline
\texttt{jigsaw} & 6 & 8 & 8 & 6 & 8\\
\hline
%\texttt{bufwriter} & 4 & 4 & 4 & 4 & 4\\
%\hline
\texttt{cryptorsa} & 1 & 1 & 2 & 1 & 2\\
\hline
\texttt{eclipse} & 37 & 42 & 45 & 43 & 53\\
\hline
\texttt{xalan} & 6 & 7 & 7 & 7 & 9\\
\hline
\texttt{lusearch} & 62 & 62 & 62 & 73 & 73\\
\hline
\end{tabular}
}
\caption{locations}
\label{tab:locations}
\end{table}

==> experimental_table_locs_distances.tex <==
\begin{table}
\parbox{.45\linewidth}{
\small
\centerline{
\begin{tabular}{|c||c|c|c|}
\hline
\textbf{Benchmark} & \textbf{Mean Distance} & \textbf{Max Distance}\\
\hline
\hline
%\texttt{array} & 0 & 0\\
%\hline
%\texttt{critical} & 10 & 16\\
%\hline
%\texttt{airtickets} & 17 & 60\\
%\hline
%\texttt{account} & 10 & 11\\
%\hline
%\texttt{pingpong} & 46 & 97\\
%\hline
%\texttt{bbuffer} & 139 & 214\\
%\hline
%\texttt{mergesort} & 939 & 1.0K\\
%\hline
%\texttt{bubblesort} & 1.0K & 3.0K\\
%\hline
%\texttt{raytracer} & 382 & 880\\
%\hline
\texttt{ftpserver} & 939 & 12K\\
%\hline
%\texttt{moldyn} & 3.0K & 10K\\
%\hline
%\texttt{derby} & 434 & 3.0K\\
\hline
\texttt{jigsaw} & 1.0K & 4.0K\\
%\hline
%\texttt{bufwriter} & 42 & 130\\
\hline
\texttt{cryptorsa} & 144K & 391K\\
\hline
\texttt{eclipse} & 11M & 53M\\
\hline
\texttt{xalan} & 2.0K & 43K\\
\hline
\texttt{lusearch} & 44M & 125M\\
\hline
\end{tabular}
}
\caption{Mean and maximum distances on races detected by $\RaceFunction$.}
\label{tab:distances}
}
\hfill
\parbox{.45\linewidth}{
\small
\centerline{
\begin{tabular}{|c||c|c|c|c|c|}
\hline
\textbf{Benchmark} &$\boldsymbol{\HB}$& $\boldsymbol{\WCP}$& $\boldsymbol{\DC}$& $\boldsymbol{\SHB}$& $\boldsymbol{\RaceFunction}$\\
\hline
\hline
%\texttt{array} & 0 & 0 & 0 & 0 & 0\\
%\hline
%\texttt{critical} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{airtickets} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{account} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{pingpong} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{bbuffer} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{mergesort} & 1 & 1 & 1 & 1 & 1\\
%\hline
%\texttt{bubblesort} & 25 & 25 & 25 & 25 & 25\\
%\hline
%\texttt{raytracer} & 3 & 3 & 3 & 3 & 3\\
%\hline
\texttt{ftpserver} & 51 & 51 & 51 & 51 & 54\\
\hline
%\texttt{moldyn} & 2 & 2 & 2 & 2 & 2\\
%\hline
%\texttt{derby} & 15 & 15 & 15 & 15 & 15\\
%\hline
\texttt{jigsaw} & 6 & 8 & 8 & 6 & 8\\
\hline
%\texttt{bufwriter} & 4 & 4 & 4 & 4 & 4\\
%\hline
\texttt{cryptorsa} & 1 & 1 & 2 & 1 & 2\\
\hline
\texttt{eclipse} & 37 & 42 & 45 & 43 & 53\\
\hline
\texttt{xalan} & 6 & 7 & 7 & 7 & 9\\
\hline
\texttt{lusearch} & 62 & 62 & 62 & 73 & 73\\
\hline
\end{tabular}
}
\caption{Number of racy locations reported by each method.}
\label{tab:locations}
}
\end{table}

==> experimental_table_race_events.tex <==
\begin{table}
\small
\centerline{
\begin{tabular}{|c|c||c|c|}
\hline
\textbf{Benchmark} & \textbf{Races}  & \textbf{Benchmark} & \textbf{Races} \\
\hline
\hline
array & 0 & ftpserver & 116\\
\hline
critical & 8 & moldyn & 9058\\
\hline
airlinetickets & 6 & derby & 39\\
\hline
account & 3 & jigsaw & 20\\
\hline
pingpong & 6 & bufwriter & 11\\
\hline
boundedbuffer & 9 & hsqldb & 848\\
\hline
mergesort & 53 & cryptorsa & 77\\
\hline
bubblesort & 909 & eclipse & 898\\
\hline
raytracer & 667 & xalan & 97\\
\hline
\end{tabular}
}
\caption{Number of races defined as race pairs $(\Event_1, \Event_2)$ discovered by $\RaceFunction$ in each benchmark.}
\label{tab:experimental_race_events}
\end{table}


==> experimental_table_races_old.tex <==

\begin{table*}
\small
\centerline{
\begin{tabular}{|c|||c|c||c|c||c|c||c|c||c|c|c|}
\hline
\textbf{Benchmark} &  \multicolumn{2}{c||}{$\boldsymbol{\HB}$}& \multicolumn{2}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{2}{c||}{$\boldsymbol{\DC}$}& \multicolumn{2}{c||}{$\boldsymbol{\SHB}$}& \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
& $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\FalseNegativesBound}$ & $\boldsymbol{\Time}$ \\
\hline
\hline
\texttt{array} & 0 & 0.30s & 0 & 0.28s & 0 & 2.12s & 0 & 0.29s & 0 & 0 & 0.13s\\
\hline
\texttt{critical} & 3 & 0.29s & 3 & 0.30s & 3 & 2.11s & 8 & 0.28s & 8 & 0 & 0.11s\\
\hline
\texttt{airtickets} & 5 & 0.32s & 5 & 0.31s & 5 & 2.10s & 6 & 0.31s & 6 & 0 & 0.09s\\
\hline
\texttt{account} & 3 & 0.31s & 3 & 0.32s & 3 & 2.12s & 3 & 0.30s & 3 & 0 & 0.10s\\
\hline
\texttt{pingpong} & 4 & 0.30s & 4 & 0.31s & 5 & 2.04s & 6 & 0.31s & 6 & 0 & 0.10s\\
\hline
\texttt{bbuffer} & 3 & 0.30s & 3 & 0.31s & 3 & 2.12s & 9 & 0.31s & 9 & 0 & 0.11s\\
\hline
\texttt{mergesort} & 2 & 0.36s & 2 & 0.41s & 29 & 2.16s & 2 & 0.37s & \textbf{53} & 0 & 0.15s\\
\hline
\texttt{bubblesort} & 305 & 0.46s & 311 & 0.54s & 478 & 2.28s & 802 & 0.62s & \textbf{909} & 0 & 2.14s\\
\hline
\texttt{raytracer} & 667 & 0.51s & 667 & 0.56s & 667 & 2.57s & 667 & 0.51s & 667 & 0 & 0.24s\\
\hline
\texttt{ftpserver} & 87 & 0.79s & 87 & 1.28s & 95 & 2.75s & 87 & 0.73s & \textbf{116} & 0 & 1.79s\\
\hline
\texttt{moldyn} & 9058 & 1.50s & 9058 & 1.81s & 9058 & 3.88s & 9058 & 1.52s & 9058 & 0 & 0.92s\\
\hline
\texttt{derby} & 38 & 8.53s & 38 & 14.54s & 38 & 15.29s & 39 & 8.32s & 39 & 0 & 7.15s\\
\hline
\texttt{jigsaw} & 15 & 17.51s & 17 & 21.80s & 17 & 40.89s & 18 & 17.93s & \textbf{20} & 0 & 12.80s\\
\hline
\texttt{bufwriter} & 11 & 48.64s & 11 & 2m0s & 11 & 2m59s & 11 & 47.71s & 11 & 0 & 2m10s\\
\hline
\texttt{cryptorsa} & 5 & 3m1s & 5 & 2m42s & 7 & 6m18s & 5 & 2m46s & \textbf{26} & 0 & 2m36s\\
\hline
\texttt{eclipse} & 378 & 8m1s & 398 & 7m0s & 465 & 14m44s & 662 & 7m11s & \textbf{898} & 1 & 1h58m\\
\hline
\texttt{xalan} & 67 & 8m58s & 68 & 8m25s & 72 & 20m12s & 89 & 9m8s & \textbf{97} & 0 & 7m56s\\
\hline
\texttt{lusearch} & 170 & 16m4s & 170 & 9m59s & 170 & 2h49m6s & 360 & 15m28s & 360 & 0 & 7m36s\\
\hline
\end{tabular}
}
\caption{Experimental comparison between $\HB$, $\WCP$, $\DC$, $\SHB$ and our $\RaceFunction$.}
\label{tab:experimental}
\end{table*}


\begin{table}
\small
\centerline{
\begin{tabular}{|c|||c|c||c|c||c|c||c|c||c|c|c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c||}{$\boldsymbol{\HB}$}& \multicolumn{2}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{2}{c||}{$\boldsymbol{\DC}$}& \multicolumn{2}{c||}{$\boldsymbol{\SHB}$}& \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
&$\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\Races}$ & $\boldsymbol{\FalseNegativesBound}$ & $\boldsymbol{\Time}$ \\
\hline
\hline
\texttt{array} & 0 & 0.30s & 0 & 0.28s & 0 & 2.12s & 0 & 0.29s & 0 & 0 & 0.13s\\
\hline
\texttt{critical} & 3 & 0.29s & 3 & 0.30s & 3 & 2.11s & 8 & 0.28s & 8 & 0 & 0.11s\\
\hline
\texttt{airtickets} & 5 & 0.32s & 5 & 0.31s & 5 & 2.10s & 6 & 0.31s & 6 & 0 & 0.09s\\
\hline
\texttt{account} & 3 & 0.31s & 3 & 0.32s & 3 & 2.12s & 3 & 0.30s & 3 & 0 & 0.10s\\
\hline
\texttt{pingpong} & 4 & 0.30s & 4 & 0.31s & 5 & 2.04s & 6 & 0.31s & 6 & 0 & 0.10s\\
\hline
\texttt{bbuffer} & 3 & 0.30s & 3 & 0.31s & 3 & 2.12s & 9 & 0.31s & 9 & 0 & 0.11s\\
\hline
\texttt{mergesort} & 2 & 0.36s & 2 & 0.41s & 29 & 2.16s & 2 & 0.37s & \textbf{53} & 0 & 0.15s\\
\hline
\texttt{bubblesort} & 305 & 0.46s & 311 & 0.54s & 478 & 2.28s & 802 & 0.62s & \textbf{909} & 0 & 2.14s\\
\hline
\texttt{raytracer} & 667 & 0.51s & 667 & 0.56s & 667 & 2.57s & 667 & 0.51s & 667 & 0 & 0.24s\\
\hline
\texttt{ftpserver} & 87 & 0.79s & 87 & 1.28s & 95 & 2.75s & 87 & 0.73s & \textbf{116} & 0 & 1.79s\\
\hline
\texttt{moldyn} & 9058 & 1.50s & 9058 & 1.81s & 9058 & 3.88s & 9058 & 1.52s & 9058 & 0 & 0.92s\\
\hline
\texttt{derby} & 38 & 8.53s & 38 & 14.54s & 38 & 15.29s & 39 & 8.32s & 39 & 0 & 7.15s\\
\hline
\texttt{jigsaw} & 15 & 17.51s & 17 & 21.80s & 17 & 40.89s & 18 & 17.93s & \textbf{20} & 0 & 12.80s\\
\hline
\texttt{bufwriter} & 11 & 48.64s & 11 & 2m0s & 11 & 2m59s & 11 & 47.71s & 11 & 0 & 2m10s\\
\hline
\texttt{cryptorsa} & 34 & 3m42s & 34 & 3m0s & 36 & 6m58s & 34 & 3m29s & \textbf{77} & 0 & 7m34s\\
\hline
\texttt{eclipse} & 378 & 8m1s & 398 & 7m0s & 465 & 14m44s & 662 & 7m11s & \textbf{897} & 1 & 1h58m42s\\
\hline
\texttt{xalan} & 67 & 8m58s & 68 & 8m25s & 72 & 20m12s & 89 & 9m8s & \textbf{97} & 0 & 7m56s\\
\hline
\texttt{lusearch} & 170 & 16m4s & 170 & 9m59s & 170 & 2h49m6s & 360 & 15m28s & 360 & 0 & 7m36s\\
\hline
\textbf{Total} & \textbf{10850} & \textbf{38m6s} & \textbf{10879} & \textbf{31m9s} & \textbf{11155} & \textbf{3h35m23s} & \textbf{11861} & \textbf{36m37s} & \textbf{12336} & \textbf{1} & \textbf{2h24m26s}\\
\hline
\end{tabular}
}
\caption{races event}
\label{tab:experimental}
\end{table}



\begin{table}
\small
\centerline{
\begin{tabular}{|c|||c|c||c|c||c|c||c|c||c|c|c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c||}{$\boldsymbol{\HB}$}& \multicolumn{2}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{2}{c||}{$\boldsymbol{\DC}$}& \multicolumn{2}{c||}{$\boldsymbol{\SHB}$}& \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
&$\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\Races}$ & $\boldsymbol{\FalseNegativesBound}$ & $\boldsymbol{\Time}$ \\
\hline
\hline
\texttt{array} & 0 & 0.30s & 0 & 0.28s & 0 & 2.12s & 0 & 0.29s & 0 & 0 & 0.13s\\
\hline
\texttt{critical} & 3 & 0.29s & 3 & 0.30s & 3 & 2.11s & 8 & 0.28s & 8 & 0 & 0.11s\\
\hline
\texttt{airtickets} & 3 & 0.32s & 3 & 0.31s & 3 & 2.10s & 4 & 0.31s & 4 & 0 & 0.09s\\
\hline
\texttt{account} & 1 & 0.31s & 1 & 0.32s & 1 & 2.12s & 1 & 0.30s & 1 & 0 & 0.10s\\
\hline
\texttt{pingpong} & 2 & 0.30s & 2 & 0.31s & 2 & 2.04s & 2 & 0.31s & 2 & 0 & 0.10s\\
\hline
\texttt{bbuffer} & 2 & 0.30s & 2 & 0.31s & 2 & 2.12s & 2 & 0.31s & 2 & 0 & 0.11s\\
\hline
\texttt{mergesort} & 1 & 0.36s & 1 & 0.41s & 2 & 2.16s & 1 & 0.37s & 2 & 0 & 0.15s\\
\hline
\texttt{bubblesort} & 81 & 0.46s & 87 & 0.54s & 118 & 2.28s & 95 & 0.62s & \textbf{121} & 0 & 2.14s\\
\hline
\texttt{raytracer} & 3 & 0.51s & 3 & 0.56s & 3 & 2.57s & 3 & 0.51s & 3 & 0 & 0.24s\\
\hline
\texttt{ftpserver} & 58 & 0.79s & 58 & 1.28s & 59 & 2.75s & 58 & 0.73s & \textbf{62} & 0 & 1.79s\\
\hline
\texttt{moldyn} & 2 & 1.50s & 2 & 1.81s & 2 & 3.88s & 2 & 1.52s & 2 & 0 & 0.92s\\
\hline
\texttt{derby} & 23 & 8.53s & 23 & 14.54s & 23 & 15.29s & 23 & 8.32s & 23 & 0 & 7.15s\\
\hline
\texttt{jigsaw} & 9 & 17.51s & 11 & 21.80s & 11 & 40.89s & 9 & 17.93s & 11 & 0 & 12.80s\\
\hline
\texttt{bufwriter} & 4 & 48.64s & 4 & 2m0s & 4 & 2m59s & 4 & 47.71s & 4 & 0 & 2m10s\\
\hline
\texttt{cryptorsa} & 5 & 3m42s & 5 & 3m0s & 7 & 6m58s & 5 & 3m29s & 7 & 0 & 7m34s\\
\hline
\texttt{eclipse} & 49 & 8m1s & 54 & 7m0s & 60 & 14m44s & 87 & 7m11s & \textbf{101} & 1 & 1h58m42s\\
\hline
\texttt{xalan} & 11 & 8m58s & 12 & 8m25s & 12 & 20m12s & 12 & 9m8s & \textbf{15} & 0 & 7m56s\\
\hline
\texttt{lusearch} & 78 & 16m4s & 78 & 9m59s & 78 & 2h49m6s & 106 & 15m28s & 106 & 0 & 7m36s\\
\hline
\textbf{Total} & \textbf{335} & \textbf{38m6s} & \textbf{349} & \textbf{31m9s} & \textbf{390} & \textbf{3h35m23s} & \textbf{422} & \textbf{36m37s} & \textbf{474} & \textbf{1} & \textbf{2h24m26s}\\
\hline
\end{tabular}
}
\caption{races codeLineLocation}
\label{tab:experimental}
\end{table}



\begin{table}
\small
\centerline{
\begin{tabular}{|c|||c|c||c|c||c|c||c|c||c|c|c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c||}{$\boldsymbol{\HB}$}& \multicolumn{2}{c||}{$\boldsymbol{\WCP}$}& \multicolumn{2}{c||}{$\boldsymbol{\DC}$}& \multicolumn{2}{c||}{$\boldsymbol{\SHB}$}& \multicolumn{3}{c|}{$\boldsymbol{\RaceFunction}$}\\
\hline
&$\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\PR}$ & $\boldsymbol{\Time}$ & $\boldsymbol{\Races}$ & $\boldsymbol{\FalseNegativesBound}$ & $\boldsymbol{\Time}$ \\
\hline
\hline
\texttt{array} & 0 & 0.30s & 0 & 0.28s & 0 & 2.12s & 0 & 0.29s & 0 & 0 & 0.13s\\
\hline
\texttt{critical} & 3 & 0.29s & 3 & 0.30s & 3 & 2.11s & 8 & 0.28s & 8 & 0 & 0.11s\\
\hline
\texttt{airtickets} & 3 & 0.32s & 3 & 0.31s & 3 & 2.10s & 4 & 0.31s & 4 & 0 & 0.09s\\
\hline
\texttt{account} & 1 & 0.31s & 1 & 0.32s & 1 & 2.12s & 1 & 0.30s & 1 & 0 & 0.10s\\
\hline
\texttt{pingpong} & 2 & 0.30s & 2 & 0.31s & 2 & 2.04s & 2 & 0.31s & 2 & 0 & 0.10s\\
\hline
\texttt{bbuffer} & 2 & 0.30s & 2 & 0.31s & 2 & 2.12s & 2 & 0.31s & 2 & 0 & 0.11s\\
\hline
\texttt{mergesort} & 1 & 0.36s & 1 & 0.41s & 2 & 2.16s & 1 & 0.37s & 2 & 0 & 0.15s\\
\hline
\texttt{bubblesort} & 6 & 0.46s & 6 & 0.54s & 3 & 2.28s & 6 & 0.62s & 6 & 0 & 2.14s\\
\hline
\texttt{raytracer} & 3 & 0.51s & 3 & 0.56s & 3 & 2.57s & 3 & 0.51s & 3 & 0 & 0.24s\\
\hline
\texttt{ftpserver} & 24 & 0.79s & 24 & 1.28s & 25 & 2.75s & 24 & 0.73s & \textbf{26} & 0 & 1.79s\\
\hline
\texttt{moldyn} & 2 & 1.50s & 2 & 1.81s & 2 & 3.88s & 2 & 1.52s & 2 & 0 & 0.92s\\
\hline
\texttt{derby} & 12 & 8.53s & 12 & 14.54s & 12 & 15.29s & 12 & 8.32s & 12 & 0 & 7.15s\\
\hline
\texttt{jigsaw} & 9 & 17.51s & 11 & 21.80s & 11 & 40.89s & 9 & 17.93s & 11 & 0 & 12.80s\\
\hline
\texttt{bufwriter} & 2 & 48.64s & 2 & 2m0s & 2 & 2m59s & 2 & 47.71s & 2 & 0 & 2m10s\\
\hline
\texttt{cryptorsa} & 5 & 3m42s & 5 & 3m0s & 7 & 6m58s & 5 & 3m29s & 7 & 0 & 7m34s\\
\hline
\texttt{eclipse} & 41 & 8m1s & 43 & 7m0s & 44 & 14m44s & 61 & 7m11s & \textbf{67} & 1 & 1h58m42s\\
\hline
\texttt{xalan} & 11 & 8m58s & 12 & 8m25s & 12 & 20m12s & 12 & 9m8s & \textbf{15} & 0 & 7m56s\\
\hline
\texttt{lusearch} & 33 & 16m4s & 33 & 9m59s & 33 & 2h49m6s & 52 & 15m28s & 52 & 0 & 7m36s\\
\hline
\textbf{Total} & \textbf{160} & \textbf{38m6s} & \textbf{165} & \textbf{31m9s} & \textbf{167} & \textbf{3h35m23s} & \textbf{206} & \textbf{36m37s} & \textbf{222} & \textbf{1} & \textbf{2h24m26s}\\
\hline
\end{tabular}
}
\caption{races codeLine}
\label{tab:experimental}
\end{table}


==> figures/dc_example.tex <==
\begin{figure}
\begin{subfigure}[b]{\textwidth}
\centering
\footnotesize
\def\rownumber{}
\begin{tabular}[b]{@{\makebox[1.2em][r]{\rownumber\space}} | l | l | l | l | l | l | l |}
\normalsize{$\mathbf{\SeqTrace_1}$} & \normalsize{$\mathbf{\SeqTrace_2}$} & \normalsize{$\mathbf{\SeqTrace_3}$} & \normalsize{$\mathbf{\SeqTrace_4}$} & \normalsize{$\mathbf{\SeqTrace_5}$} & \normalsize{$\mathbf{\SeqTrace_6}$} & \normalsize{$\mathbf{\SeqTrace_7}$}
\gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\
\hline
$\Acquire(\ell_1)$ & & & & & & \\
$\Sync(s_1)$ & & & & & & \\
& $\Acquire(\ell_2)$ & & & & & \\
& $\Sync(s_2)$ & & & & & \\
& $\Sync(s_3)$ & & & & & \\
& & $\Acquire(\ell_3)$ & & & & \\
& & $\Sync(s_4)$ & & & & \\
& $\Sync(s_1)$ & & & & & \\
& $\Sync(s_4)$ & & & & & \\
& $\Release(\ell_2)$ & & & & & \\
& & & $\Acquire(\ell_2)$ & & & \\
& & & $\Sync(s_5)$ & & & \\
& & & $\Sync(s_6)$ & & & \\
& & $\Sync(s_2)$ & & & & \\
& & $\Sync(s_5)$ & & & & \\
& & $\Release(\ell_3)$ & & & & \\
& & & & $\Acquire(\ell_3)$ & &\\
& & & & $\Sync(s_7)$ & & \\
& & & & $\Sync(s_8)$ & & \\
& & & $\Sync(s_8)$ & & & \\
& & & $\Release(\ell_2)$ & & & \\
& & & & $\Sync(s_6)$ & & \\
& & & & $\Sync(s_3)$ & & \\
& & & & $\Release(\ell_3)$ & & \\
$\mathbf{\Write(x)}$ & & & & & & \\
$\Release(\ell_1)$ & & & & & & \\
& & & & & $\Acquire(\ell_1)$ & \\
& & & & & $\Sync(s_{9})$ & \\
& & & & & $\Sync(s_{7})$ & \\
& & & & & $\Release(\ell_1)$ & \\
& & & & & & $\Sync(s_{9})$\\
& & & & & & $\mathbf{\Read(x)}$ \\
\hline
\end{tabular}
\caption{Is $(\Event_{25}, \Event_{32})$ a race?}
\label{subfig:dc_example}
\end{subfigure}
\end{figure}


\begin{figure}\ContinuedFloat
\begin{subfigure}[b]{\textwidth}
\centering
\footnotesize
\def\rownumber{}
\begin{tabular}[b]{@{\makebox[1.2em][r]{\rownumber\space}} | l | l | l | l | l | l | l |}
\normalsize{$\mathbf{\SeqTrace_1}$} & \normalsize{$\mathbf{\SeqTrace_2}$} & \normalsize{$\mathbf{\SeqTrace_3}$} & \normalsize{$\mathbf{\SeqTrace_4}$} & \normalsize{$\mathbf{\SeqTrace_5}$} & \normalsize{$\mathbf{\SeqTrace_6}$} & \normalsize{$\mathbf{\SeqTrace_7}$}
\gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\
\hline
& & & & $\Acquire(\ell_3)$ & &\\
& & & & $\Sync(s_7)$ & & \\
& & & & & $\Acquire(\ell_1)$ & \\
& & & & & $\Sync(s_{9})$ & \\
& & & & & $\Sync(s_{7})$ & \\
& & & & & $\Release(\ell_1)$ & \\
$\Acquire(\ell_1)$ & & & & & & \\
$\Sync(s_1)$ & & & & & & \\
& & & $\Acquire(\ell_2)$ & & & \\
& & & $\Sync(s_5)$ & & & \\
& & & $\Sync(s_6)$ & & & \\
& & & & $\Sync(s_8)$ & & \\
& & & $\Sync(s_8)$ & & & \\
& & & $\Release(\ell_2)$ & & & \\
& $\Acquire(\ell_2)$ & & & & & \\
& $\Sync(s_2)$ & & & & & \\
& $\Sync(s_3)$ & & & & & \\
& & & & $\Sync(s_6)$ & & \\
& & & & $\Sync(s_3)$ & & \\
& & & & $\Release(\ell_3)$ & & \\
& & $\Acquire(\ell_3)$ & & & & \\
& & $\Sync(s_4)$ & & & & \\
& $\Sync(s_1)$ & & & & & \\
& $\Sync(s_4)$ & & & & & \\
& $\Release(\ell_2)$ & & & & & \\
& & $\Sync(s_2)$ & & & & \\
& & $\Sync(s_5)$ & & & & \\
& & $\Release(\ell_3)$ & & & & \\
& & & & & & $\Sync(s_{9})$\\
$\mathbf{\Write(x)}$ & & & & & & \\
& & & & & & $\mathbf{\Read(x)}$ \\
\hline
\end{tabular}
\caption{The witness trace as constructed by $\RaceFunction$.}
\label{subfig:dc_example_witness}
\end{subfigure}
\caption{The example of~\cite{Roemer18} adapted to our setting (\protect\cref{subfig:dc_example}) and the witness trace as constructed by $\RaceFunction$ (\protect\cref{subfig:dc_example_witness}).}
\label{fig:dc_example}
\end{figure}

==> figures/motivating_old.tex <==
\begin{figure}[!h]
\begin{subfigure}[b]{0.4\textwidth}
\centering
\footnotesize
\def\rownumber{}
\begin{tabular}[b]{@{\makebox[1.2em][r]{\rownumber\space}} | l | l |}
\normalsize{$\mathbf{\SeqTrace_1}$} & \normalsize{$\mathbf{\SeqTrace_2}$}
\gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\
\hline
$\Acquire(\ell)$ & \\
$\mathbf{\Write(x)}$ & \\
$\Release(\ell)$ & \\
& $\Acquire(\ell)$  \\
& $\Write(x)$  \\
& $\Release(\ell)$  \\
& $\mathbf{\Read(x)}$\\
\hline
\end{tabular}
\caption{Is $(\Event_2, \Event_7)$ a race?}
\label{subfig:motivating_incomplete1}
\end{subfigure}
%\begin{subfigure}[b]{0.25\textwidth}
%\centering
%\footnotesize
%\def\rownumber{}
%\begin{tabular}[b]{@{\makebox[1.2em][r]{\rownumber\space}} | l | l | l |}
%\normalsize{$\mathbf{\SeqTrace_1}$} & \normalsize{$\mathbf{\SeqTrace_2}$} & \normalsize{$\mathbf{\SeqTrace_3}$}
%\gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\
%\hline
%$\mathbf{\Write(x)}$ & & \\
%$\Acquire(\ell_1)$ & & \\
%$\Write(y)$ & & \\
%$\Release(\ell_1)$ & &\\
%& $\Acquire(\ell_1)$ & \\
%& $\Read(y)$ & \\
%& $\Release(\ell_1)$ & \\
%& $\Acquire(\ell_2)$ & \\
%& $\Release(\ell_2)$ & \\
%& & $\Acquire(\ell_2)$ \\
%& & $\Release(\ell_2)$ \\
%& & $\mathbf{\Read(x)}$\\
%%$\Acquire(\ell_1)$ &  & \\
%%$\Write(x)$ &  & \\
%%$\Release(\ell_1)$ & &\\
%%& $\Acquire(\ell_1)$ & \\
%%& $\Read(x)$ & \\
%%& $\Release(\ell_1)$ &  \\
%%& $\Acquire(\ell_2)$ & \\
%%& $\Release(\ell_2)$ & \\
%%& & $\Acquire(\ell_2)$ \\
%%& & $\Read(x)$ \\
%%& & $\Release(\ell_2)$ \\
%\hline
%\end{tabular}
%\caption{}
%\label{subfig:motivating_incomplete2}
%\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
\centering
\footnotesize
\def\rownumber{}
\begin{tabular}[b]{@{\makebox[1.2em][r]{\rownumber\space}} | l | l | l |}
\normalsize{$\mathbf{\SeqTrace_1}$} & \normalsize{$\mathbf{\SeqTrace_2}$} & \normalsize{$\mathbf{\SeqTrace_3}$}
\gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\
\hline
$\Acquire(\ell_1)$ & & \\
$\Release(\ell_1)$ & & \\
$\mathbf{\Write(x)}$ & & \\
$\Acquire(\ell_1)$ & & \\
$\Release(\ell_1)$ & & \\
& $\Acquire(\ell_1)$ & \\
& $\Acquire(\ell_2)$ & \\
& $\Write(y)$ & \\
& $\Release(\ell_2)$ & \\
& $\Release(\ell_1)$ & \\
& & $\Acquire(\ell_2)$ \\
& & $\Read(y)$ \\
& & $\Release(\ell_2)$ \\
& & $\mathbf{\Read(x)}$\\
\hline
\end{tabular}
\caption{Is $(\Event_3, \Event_{14})$ a race?}
\label{subfig:motivating_incomplete2}
\end{subfigure}
\caption{
Examples in which $\HB$, $\WCP$ and $\DC$ are incomplete.
(\protect\subref{subfig:motivating_incomplete1})~A race $(\Event_2, \Event_7)$ missed by $\HB$, $\WCP$ and $\DC$.
(\protect\subref{subfig:motivating_incomplete2})~A race $(\Event_2, \Event_{10})$ missed by $\HB$, $\WCP$ and $\DC$ (after vindication).
}
\label{fig:motivating}
\end{figure}


==> outline.tex <==
%\subsection{Organization and Outline}\label{subsec:outline}
\smallskip\noindent{\bf Organization and outline.}
We briefly summarize the organization of the paper, which also gives an outline of our approach.
\begin{compactenum}
\item[In \cref{sec:po}]
we develop concepts related to partial orders.
We define the notion of trace-closure of a partial order and show that
(i)~the closure can be computed efficiently, and
(ii)~certain trace-closed partial orders are always linearizable to valid traces.
Conceptually, the partial orders considered in (ii)~are weaker than other types of partial orders constructed in the literature, 
which allows us to detect more races.
\item[In \cref{sec:decision}]
We present our algorithm $\RaceDecision$ for the decision problem of race detection, i.e, deciding whether an event $(\Event_1, \Event_2)$ constitutes a predictable race of an input trace $\Trace$.

\item[In \cref{sec:function}]
We also develop sound criteria for over-approximating the set of false negatives.

\item[In \cref{sec:experiments}]
we perform an experimental evaluation of our algorithm $\RaceFunction$ on a standard set of benchmark traces,
and compare its performance against state-of-the-art fast and sound methods for dynamic race detection.
\end{compactenum}




==> related_work.tex <==
\subsection{Other Related Work}\label{subsec:related_work}
